Drell-Yan at the Electron-Ion Collider

The photon is arguably the most universally important particle across all fields of physics. Despite its status as a fundamental particle, at high energies the photon can be seen as a hadronic source of partons. The partonic content of the photon is very poorly constrained compared to that of the proton, with photon PDF uncertainties typically one or two orders of magnitude larger than their proton counterparts, despite the fact that its source, the $\gamma\to q\bar{q}$ splitting, is perturbatively calculable. The high luminosity, excellent particle identification, and far-backward electron tagging capabilities of the Electron-Ion Collider make it an ideal environment for studying photon parton distribution functions. Similar to the $p+p$ or $\pi+p$ systems, photoproduction at the EIC can be thought of as two parton distributions colliding. One of the most powerful processes in such collisions is production of lepton pairs, i.e. $h+p\rightarrow l^+l^-+X$, known as the Drell--Yan process. This process has the ability to access for the first time the transverse-momentum-dependent parton distributions of the photon. The transversely polarized proton beam of the EIC additionally provides a possible means of accessing the transversity distribution of the proton without relying on fragmentation functions.

==> defs.tex <==
%===============================================================================
% defs.tex — common macros for physics papers
%===============================================================================
\ProvidesFile{defs.tex}[2025/06/21 v1.0 Common physics & formatting macros]

%% units
\newcommand{\GeV}{\ensuremath{\mathrm{GeV}}\xspace}
\newcommand{\GeVsq}{\ensuremath{\mathrm{GeV}^2}\xspace}
\newcommand{\MeV}{\ensuremath{\mathrm{MeV}}\xspace}
\newcommand{\TeV}{\ensuremath{\mathrm{TeV}}\xspace}

%% kinematic variables
\newcommand{\qsq}{\ensuremath{Q^2}\xspace}
\newcommand{\xbj}{\ensuremath{x_{\mathrm{Bj}}}\xspace}
\newcommand{\eps}{$\varepsilon$\xspace}

%% processes & reactions
\newcommand{\epem}{\ensuremath{e^+e^-}\xspace}
\newcommand{\epp}{\ensuremath{e^+p}\xspace}
\newcommand{\emp}{\ensuremath{e^-p}\xspace}
\newcommand{\eep}{\ensuremath{e^\pm p}\xspace}
\newcommand{\epphi}{\ensuremath{e + p \to e + p + \phi}\xspace}

%% structure functions & form-factors
\newcommand{\Fthree}{\ensuremath{F_3^{\gamma Z}}\xspace}
\newcommand{\GE}{\ensuremath{G_E}\xspace}
\newcommand{\GM}{\ensuremath{G_M}\xspace}

%% math shortcuts
\newcommand{\order}[1]{\ensuremath{\mathcal{O}\!\bigl(#1\bigr)}\xspace}
\newcommand{\dd}{\ensuremath{\,\mathrm{d}}\xspace}

%% styling & formatting
\newcommand{\figref}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\secref}[1]{Sec.~\ref{#1}\xspace}
\newcommand{\eqnref}[1]{Eq.~\eqref{#1}\xspace}

%===============================================================================

